The Taboo Trap: Behavioural Detection of Adversarial Samples

Deep Neural Networks (DNNs) have become a powerful toolfor a wide range of problems. Yet recent work has found an increasing variety of adversarial samplesthat can fool them. Most existing detection mechanisms against adversarial attacksimpose significant costs, either by using additional classifiers to spot adversarial samples, or by requiring the DNN to be restructured. In this paper, we introduce a novel defence. We train our DNN so that, as long as it is workingas intended on the kind of inputs we expect, its behavior is constrained, in that some set of behaviors are taboo. If it is exposed to adversarial samples, they will often cause a taboo behavior, which we can detect. Taboos can be both subtle and diverse, so their choice can encode and hide information. It is a well-established design principle that the security of a system should not depend on the obscurity of its design, but on some variable (the key) which can differ between implementations and bechanged as necessary. We discuss how taboos can be used to equip a classifier with just such a key, and how to tune the keying mechanism to adversaries of various capabilities. We evaluate the performance of a prototype against a wide range of attacks and show how our simple defense can defend against cheap attacks at scale with zero run-time computation overhead, making it a suitable defense method for IoT devices.

==> sections/__latexindent_temp.tex <==
\begin{table}[!h]
\adjustbox{max width=\linewidth}{%
\centering
\begin{tabular}{@{}l|l|l|l|ll|l|@{}}
\toprule
Technique& $\theta$ & FGSM & DeepFool & New MACs & as \% & New Params \\ \midrule
% Taboo Trap & $f=1^{st}$ max percentile & 0.99 & 0.14 & 0 & 0 & 0\\ \midrule
% MagNet & & 1.0 & 1.0 & 137592 & 6 & 297 \\ \midrule
% \multirow{2}{*}{Metzen et al.}& 1 layer, DeepFool & 0.92  & 0.82  & $\sim 34810489$ & 1518 & 5945367 \\
% & 3 layers, DeepFool & 0.98  & 0.92  & $\sim 21767179$ & 949 & 4861597 \\
Taboo Trap & $P_{1}$ & 0.99 & 0.14 & \textbf{0} & \textbf{0} & \textbf{0}\\ \midrule
MagNet & & 1.0 & 1.0 & 190K & 20 & 297 \\ \midrule
\multirow{2}{*}{SafetyNet et al.}& 1 layer & 0.92  & 0.82  & 34.81M & 3622 & 5,95M \\
& 3 layers & 0.98  & 0.92  & 21.77M & 2265 & 4.86M \\
\bottomrule
\end{tabular}}
\caption{LeNet5 has 961K multiply-accumulate operations (MACs) and 17.75K parameters without defenses. SafetyNet is trained on the DeepFool adversarial samples. $P_{i}$ refers to the $i$th-percentile. FGSM $\epsilon=0.8$ is used. Overhead for MagNet is only calculated over the detector.}
\label{tab:len-act}
\end{table}
